Hypergeometric SLE: Conformal Markov Characterization and Applications

This article pertains to the classification of pairs of simple random curves with conformal Markov property and symmetry. We give the complete classification of such curves: conformal Markov property and symmetry single out a two-parameter family of random curves---Hypergeometric SLE---denoted by hSLE$_{\kappa}(\nu)$ for $\kappa\in (0,4]$ and $\nu<\kappa-6$. The proof relies crucially on Dub\'edat's commutation relation [Dub07] and a uniqueness result proved in [MS16b]. The classification indicates that hypergeometric SLE is the only possible scaling limit of the interfaces in critical lattice models (conjectured or proved to be conformal invariant) in topological rectangles with alternating boundary conditions. We also prove various properties of hSLE: continuity, reversibility, target-independence, and conditional law characterization. As by-products, we give two applications of these properties. The first one is about the critical Ising interfaces. We prove the convergence of the Ising interface in rectangles with alternating boundary conditions. This result was first proved by Izyurov in [Izy15], but our proof is new which is based on the properties of hSLE. The second application is the existence of the so-called pure partition functions of multiple SLEs. Such existence was proved for $\kappa\in (0,8)\setminus \mathbb{Q}$ in [KP16], and it was later proved for $\kappa\in (0,4]$ in [PW17]. We give a new proof of the existence for $\kappa\in (0,6]$ using the properties of hSLE.

==> tex/purepartitionfunctions.tex <==






We will prove the existence in Proposition~\ref{prop::purepartition_existence} by induction on $N$. It is immediate to check the existence for $N=1$ and $N=2$. 
When $N=1$, for $x<y$ and  
$\vcenter{\hbox{\includegraphics[scale=0.3]{figures/link-0.pdf}}} = \{\{1,2\}\}$,
\[ \PartF_{\vcenter{\hbox{\includegraphics[scale=0.2]{figures/link-0.pdf}}}}(x,y) 
= (y-x)^{-2h} . \]
When $N=2$, we obtain 
for $\vcenter{\hbox{\includegraphics[scale=0.3]{figures/link-2.pdf}}} = \{\{1,4\}, \{2,3\} \}$ 
and $\vcenter{\hbox{\includegraphics[scale=0.3]{figures/link-1.pdf}}} = \{\{1,2\}, \{3,4\}\}$, 
and for $x_1<x_2<x_3<x_4$,
\begin{align*}
\PartF_{\vcenter{\hbox{\includegraphics[scale=0.2]{figures/link-2.pdf}}}} (x_1,x_2,x_3,x_4)
= \; & (x_4-x_1)^{-2h}(x_3-x_2)^{-2h}z^{2/\kappa}F(z) , \\ 
\PartF_{\vcenter{\hbox{\includegraphics[scale=0.2]{figures/link-1.pdf}}}} (x_1,x_2,x_3,x_4)
= \; &  (x_2-x_1)^{-2h}(x_4-x_3)^{-2h}(1-z)^{2/\kappa}F(1-z),
\end{align*}
where $z$ is the cross-ratio and $F$ is the hypergeometric function as in~\eqref{eqn::hSLE_partition}:
\[z=\frac{(x_2-x_1)(x_4-x_3)}{(x_4-x_2)(x_3-x_1)},\quad F(z):=\hF\left(\frac{4}{\kappa}, 1-\frac{4}{\kappa}, \frac{8}{\kappa}; z\right).\]

{\color{blue}The boundary Poisson kernel has monotonicity: suppose $(\Omega; x, y)$ is a Dobrushin domain such that $x,y$ lie on analytic segments of $\partial\Omega$, and suppose $U\subset\Omega$ is simply connected and agrees with $\Omega$ is neighborhoods of $x$ and $y$, then 
\begin{equation}\label{eqn::poisson_mono}
H_{U}(x,y)\le H_{\Omega}(x,y).
\end{equation}
As a consequence, we have the monotonicity of $\LB_{\alpha}$: suppose $(\Omega; x_1, \ldots, x_{2N})$ is a polygon such that $x_1, \ldots, x_{2N}$ lie on analytic segments of $\partial\Omega$, and suppose $U\subset\Omega$ is simply connected and agrees with $\Omega$ in neighborhoods of $\{x_1, \ldots, x_{2N}\}$, then, for any $\alpha\in\LP_N$,
\begin{equation}\label{eqn::balpha_mono}
\LB_{\alpha}(U; x_1, \ldots, x_{2N})\le \LB_{\alpha}(\Omega; x_1, \ldots, x_{2N}),
\end{equation}
because $h\ge 0$ when $\kappa\le 6$. 
}
Suppose the collection of pure partition functions exists up to $N$, and we consider $\LP_{N+1}$. Suppose $\alpha=\{\{a_1, b_1\}, \ldots, \{a_{N+1}, b_{N+1}\}\}$, and we may assume $a_j<b_j$ for all $1\le j\le N+1$. Consider the polygon $(\Omega; x_1, \ldots, x_{2N+2})$. 
For $1\le k\le N+1$, let $\eta_k$ be an $\SLE_{\kappa}$ in $\Omega$ from $x_{a_k}$ to $x_{b_k}$. Consider the set $\Omega\setminus\eta_k$, we denote by $D_k^R$  the connected component having $(x_{a_k+1}x_{b_k-1})$ on the boundary, and denote by $D_k^L$ the connected component having $(x_{b_k+1}x_{a_k-1})$ on the boundary, {\color{red}see Figure~\ref{???}}.
The link $\{a_k, b_k\}$ divides the link pattern $\alpha$ into two sub-link patterns, connecting $\{a_k+1, \ldots, b_k-1\}$ and $\{b_k+1, \ldots, a_{k}-1\}$ respectively. After relabelling the indices, we denote these two link patterns by $\alpha_k^R$ and $\alpha_k^L$. 

As the pure partition functions exist up to $N$, the following two functions are well-defined: 
\[\PartF_{\alpha_k^R}(D_k^R; x_{a_k+1}, x_{a_k+2}, \ldots, x_{b_k-1}),\quad \PartF_{\alpha_k^L}(D_k^L; x_{b_k+1}, x_{b_k+2},\ldots, x_{a_k-1}). \] 
Then, we define 
\begin{align}\label{eqn::purepartition_cascade_def}
&\PartF_{\alpha}^{(k)}(\Omega; x_1, \ldots, x_{2N+2})\notag\\
&=H_{\Omega}( x_{a_k}, x_{b_k})^h\E\left[\PartF_{\alpha_k^R}(D_k^R; x_{a_k+1}, \ldots, x_{b_k-1})\times\PartF_{\alpha_k^L}(D_k^L; x_{b_k+1},\ldots, x_{a_k-1})\right].
\end{align}
At this point, the definition of $\PartF_{\alpha}^{(k)}$ depends on the choice of $k\in\{1, \ldots, N+1\}$, but we will show later that, in fact, the function defined in~\eqref{eqn::purepartition_cascade_def} does not depend on the choice of $k$. 

\begin{lemma}\label{lem::purepartition_cascade_COV}
The function defined in~\eqref{eqn::purepartition_cascade_def} satisfies COV~\eqref{eqn::purepartition_COV}.
\end{lemma}
\begin{proof}
This is true because: (a) $\SLE_{\kappa}$ is conformally invariant; (b) the boundary Poisson kernel is conformally covariant; (c) the pure partition functions $\PartF_{\alpha_k^R}$ and $\PartF_{\alpha_k^L}$ are conformally covariant by the induction hypothesis. 
\end{proof}

\begin{lemma}\label{lem::purepartition_cascade_ASY}
The function defined in~\eqref{eqn::purepartition_cascade_def} satisfies ASY~\eqref{eqn::purepartition_ASY_polygon}. 
\end{lemma}
\begin{proof}
In order to prove ASY~\eqref{eqn::purepartition_ASY_polygon}, we need to check the following cases: Case (a). $\{a_k, b_k\}=\{j, j+1\}$; Case (b). $a_k=j$ and $b_k\neq j+1$. The cases $\#\{a_k, b_k\}\cap\{j,j+1\}=1$ can be proved similarly; Case (c). $\{a_k, b_k\}\cap\{j, j+1\}=\emptyset$. 

\smallbreak
Case (a). Suppose $\{a_k, b_k\}=\{j, j+1\}$. Note that $\eta_k$ is the $\SLE_{\kappa}$ in $\HH$ from $x_j$ to $x_{j+1}$. In this case, $\alpha_k^R=\emptyset$ and $\alpha_k^L=\hat{\alpha}:=\alpha\removal\{j,j+1\}$. 
Then we have 
\begin{align*}
\PartF_{\alpha}^{(k)}(\Omega; x_1, \ldots, x_{2N+2})=H_{\Omega}(x_{j}, x_{j+1})^h\E\left[\PartF_{\hat{\alpha}}(D_k^L; x_{j+2}, \ldots, x_{j-1})\right].
\end{align*}
By the induction hypothesis and~\eqref{eqn::balpha_mono}, we have
\[\PartF_{\hat{\alpha}}(D_k^L; x_{j+2}, \ldots, x_{j-1})
\le \LB_{\hat{\alpha}}(D_k^L; x_{j+2}, \ldots, x_{j-1})
\le \LB_{\hat{\alpha}}(\Omega; x_{j+2}, \ldots, x_{j-1}).\]
Bounded convergence theorem gives 
\begin{align*}
\lim_{x_j, x_{j+1}\to \xi}\frac{\PartF_{\alpha}^{(k)}(\Omega; x_1, \ldots, x_{2N+2})}{H_{\Omega}(x_{j}, x_{j+1})^h}=\lim_{x_j, x_{j+1}\to \xi}\E\left[\PartF_{\hat{\alpha}}(D_k^L; x_{j+2}, \ldots, x_{j-1})\right]=\PartF_{\hat{\alpha}}(\Omega; x_{j+2}, \ldots, x_{j-1}).
\end{align*}

\smallbreak
Case (b). $a_k=j$ and $b_k\neq j+1$. In this case, we have 
\begin{align*}
&\frac{\PartF_{\alpha}^{(k)}(\Omega; x_1, \ldots, x_{2N+2})}{H_{\Omega}(x_j, x_{j+1})^h}\\
&=H_{\Omega}( x_{a_k}, x_{b_k})^h\E\left[\frac{\PartF_{\alpha_k^R}(D_k^R; x_{a_k+1}, \ldots, x_{b_k-1})}{H_{\Omega}(x_j, x_{j+1})^h}\times\PartF_{\alpha_k^L}(D_k^L; x_{b_k+1},\ldots, x_{a_k-1})\right].
\end{align*} 
By the induction hypothesis and~\eqref{eqn::balpha_mono}, we have 
\begin{align*}
\PartF_{\alpha_k^L}(D_k^L; x_{b_k+1},\ldots, x_{a_k-1})
&\le \LB_{\alpha_k^L}(\Omega; x_{b_k+1},\ldots, x_{a_k-1});\\
\frac{\PartF_{\alpha_k^R}(D_k^R; x_{a_k+1}, \ldots, x_{b_k-1})}{H_{\Omega}(x_j, x_{j+1})^h}
&\le \frac{\LB_{\alpha_k^R}(\Omega; x_{a_k+1}, \ldots, x_{b_k-1})}{H_{\Omega}(x_j, x_{j+1})^h}\to 0,\quad\text{as }x_j, x_{j+1}\to \xi. 
\end{align*}
Thus,
\[\lim_{x_j, x_{j+1}\to \xi}\frac{\PartF_{\alpha}^{(k)}(\Omega; x_1, \ldots, x_{2N+2})}{H_{\Omega}(x_j, x_{j+1})^h}=0.\]

\smallbreak
Case (c). $\{a_k, b_k\}\cap\{j, j+1\}=\emptyset$. We may assume $a_k<j<j+1<b_k$. In this case, we have 
\begin{align*}
&\frac{\PartF_{\alpha}^{(k)}(\Omega; x_1, \ldots, x_{2N+2})}{H_{\Omega}(x_j, x_{j+1})^h}\\
&=H_{\Omega}( x_{a_k}, x_{b_k})^h\E\left[\frac{\PartF_{\alpha_k^R}(D_k^R; x_{a_k+1}, \ldots, x_{b_k-1})}{H_{\Omega}(x_j, x_{j+1})^h}\times\PartF_{\alpha_k^L}(D_k^L; x_{b_k+1},\ldots, x_{a_k-1})\right].
\end{align*} 
By the induction hypothesis and~\eqref{eqn::balpha_mono}, we have
\begin{align*}
\PartF_{\alpha_k^L}(D_k^L; x_{b_k+1},\ldots, x_{a_k-1})
&\le \LB_{\alpha_k^L}(\Omega; x_{b_k+1},\ldots, x_{a_k-1});\\
\frac{\PartF_{\alpha_k^R}(D_k^R; x_{a_k+1}, \ldots, x_{b_k-1})}{H_{\Omega}(x_j, x_{j+1})^h}
&\le \frac{\LB_{\alpha_k^R}(\Omega; x_{a_k+1}, \ldots, x_{b_k-1})}{H_{\Omega}(x_j, x_{j+1})^h}\to 0,\quad\text{as }x_j, x_{j+1}\to \xi. 
\end{align*}

\end{proof}




